LLM Post-Training: A Deep Dive into Reasoning Large Language Models

Large Language Models (LLMs) have transformed the natural language processing landscape and brought to life diverse applications. Pretraining on vast web-scale data has laid the foundation for these models, yet the research community is now increasingly shifting focus toward post-training techniques to achieve further breakthroughs. While pretraining provides a broad linguistic foundation, post-training methods enable LLMs to refine their knowledge, improve reasoning, enhance factual accuracy, and align more effectively with user intents and ethical considerations. Fine-tuning, reinforcement learning, and test-time scaling have emerged as critical strategies for optimizing LLMs performance, ensuring robustness, and improving adaptability across various real-world tasks. This survey provides a systematic exploration of post-training methodologies, analyzing their role in refining LLMs beyond pretraining, addressing key challenges such as catastrophic forgetting, reward hacking, and inference-time trade-offs. We highlight emerging directions in model alignment, scalable adaptation, and inference-time reasoning, and outline future research directions. We also provide a public repository to continually track developments in this fast-evolving field: https://github.com/mbzuai-oryx/Awesome-LLM-Post-training.

==> figures/rl_llm_fig.tex <==
\begin{figure}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[
    node distance=3.5cm and 2.5cm,
    >=Stealth,
    align=center,
    font=\footnotesize
]

%--- Node Styles -------------------------------------------------%
\tikzstyle{boxEnv} = [
    rectangle, 
    rounded corners, 
    draw=black, 
    fill=green!20, 
    minimum width=3.5cm, 
    minimum height=1.4cm, 
    text centered
]
\tikzstyle{boxAgent} = [
    rectangle, 
    rounded corners, 
    draw=black, 
    fill=blue!20, 
    minimum width=3.5cm, 
    minimum height=1.4cm, 
    text centered
]
\tikzstyle{boxReward} = [
    rectangle, 
    rounded corners, 
    draw=black, 
    fill=red!20, 
    minimum width=3.5cm, 
    minimum height=1.4cm, 
    text centered
]
\tikzstyle{arrow} = [->, thick]

%--- Nodes -------------------------------------------------------%
\node[boxEnv] (env) {\textbf{Environment}\\(Prompt, Context)};
\node[boxAgent, right=30mm of env] (agent) {\textbf{Agent}\\(LLM as Policy Network, $\theta$)};
\node[boxReward, below=15mm of env] (reward) {\textbf{Reward}\\(Feedback, Score)};

%--- Arrows (Showing Direct Interaction) -------------%
% \draw[arrow] (env) -- node[midway, above] {State (Text Context)} (agent);
% \draw[arrow] (agent.west) to[out=180, in=0] node[midway, below] {Token Generation} (env.east);
% \draw[arrow] (env.south) -- node[midway, left] {Evaluates Tokens} (reward.north);
% \draw[arrow] (reward.east) -- node[midway, below] {$\theta$ Update} (agent.south);
%--- Arrows (Adjusted for Vertical Offsets) -------------%
\draw[arrow] (env.east)++(0,0.1) to[out=10, in=170]  node[midway, above] {State (Text Context)} (agent.west);
\draw[arrow] (agent.west)++(0,-0.1) to[out=190, in=-10] node[midway, below] {Token Generation} (env.east);
\draw[arrow] (env.south) -- node[midway, left] {Evaluates Tokens} (reward.north);
\draw[arrow] (reward.east) to[out=0, in=270] node[midway, right] {$\qquad\theta$ Update} (agent.south);


\end{tikzpicture}%
}
\caption{An illustration of reinforcement learning in LLMs, where the environment provides inputs in the form of user prompts and conversation context, and the agent generates tokens as actions, which go back to the environment for evaluation, producing rewards that update the agent’s policy.}
\label{fig:rl_llm_simple}
\end{figure}





% Komal %%%%%%%%%%%%%%%%%%%%%%%


==> tables/datasets_train.tex <==
\begin{table*}[htbp]
\centering
\caption{Prominent Datasets for Training and Fine-Tuning Large Language Models}
\label{tab:llm_datasets}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lcccc}
\toprule
\rowcolor[HTML]{EFEFEF}
\textbf{Dataset} & \textbf{Developer} & \textbf{Domain} & \textbf{Size} & \textbf{Languages} \\
\midrule
\textbf{The Pile}~\cite{gao2020pile, biderman2022datasheet} & EleutherAI & General & 825 GB & English \\
\rowcolor[HTML]{F7F7F7}
\textbf{CulturaX}~\cite{nguyen-etal-2024-culturax} & University of Oregon NLP Group & Multilingual & 6.3T tokens & 167 languages \\
\textbf{RedPajama}~\cite{weber2024redpajama} & Together AI & General & 1.2T tokens & English \\
\rowcolor[HTML]{F7F7F7}
\textbf{BookCorpus}~\cite{bandy2021addressing} & University of Toronto & Literature & 985M words & English \\
\textbf{OpenSubtitles}~\cite{lison2016opensubtitles2016} & OpenSubtitles.org & Dialogue & 24 GB & Multiple \\
\rowcolor[HTML]{F7F7F7}
\textbf{LAION-5B}~\cite{schuhmann2022laion5bopenlargescaledataset} & LAION & Multimodal & 5.85B image-text pairs & Multiple \\
\textbf{Dolma}~\cite{dolma}~\cite{} & Allen Institute for AI & General & 3T tokens & English \\
\rowcolor[HTML]{F7F7F7}
\textbf{Zyda}~\cite{tokpanov2024zyda} & OpenAI & General & 1.3T tokens & English \\
\textbf{Common Crawl}~\cite{turski2023ccpdfbuildinghighquality} & Common Crawl Foundation & Web & Multiple PB & Multiple \\
\rowcolor[HTML]{F7F7F7}
\textbf{Wikipedia}~\cite{wikidump} & Wikimedia Foundation & Encyclopedia & 20 GB & Multiple \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/key_terms.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{0.9} % Reduce row height
\small % Use small font instead of scriptsize
\resizebox{\columnwidth}{!}{ % Adjusts the table to fit the column width
\begin{tabular}{l c p{3.5cm}}
\toprule
\textbf{Key Terms} & \textbf{Representation} & \textbf{Mathematical Concept} \\
\midrule
State & \( s_t \) & Decision Theory \\
Action & \( a_t \) & Decision Theory \\
Policy & \( \pi_{\theta} \) & Optimization \\
Reward Function & \( R \) & Reinforcement Learning \\
Return & \( G_t \) & Reinforcement Learning \\
Value Function & \( V^\pi \) & Dynamic Programming \\
Q-Function & \( Q^\pi \) & Dynamic Programming \\
Advantage Function & \( A \) & Reinforcement Learning \\
Entropy & \( H(\pi) \) & Information Theory \\
KL Divergence & \( D_{KL} \) & Probability Theory \\
Fine-Tuning & \( \Delta \theta \) & Optimization \\
LoRA & \( \Delta \mathbf{W} \) & Optimization \\
Prompt Engineering & \( P \) & NLP \\
RAG & \( R_{t} \) & Information Retrieval \\
Scaling & \( S \) & Complexity Theory \\
Search Techniques & \( \text{Search}(s_t) \) & Search Algorithms \\
Test-Time Adaptation & \( \theta^* \) & Machine Learning \\
Distribution Alignment & \( D_{align} \) & Statistical Learning \\
Entropy Regularization & \( H_{reg}(\pi) \) & Reinforcement Learning \\
\bottomrule
\end{tabular}
}
\caption{Key terminology and notations for RL-enhanced LLMs, Test-Time Scaling, and Fine-Tuning.}
\label{tab:key-terms-rl-llm}
\end{table}

